Compositional Inference Metaprogramming with Convergence Guarantees

Inference metaprogramming enables effective probabilistic programming by supporting the decomposition of executions of probabilistic programs into subproblems and the deployment of hybrid probabilistic inference algorithms that apply different probabilistic inference algorithms to different subproblems. We introduce the concept of independent subproblem inference (as opposed to entangled subproblem inference in which the subproblem inference algorithm operates over the full program trace) and present a mathematical framework for studying convergence properties of hybrid inference algorithms that apply different Markov-Chain Monte Carlo algorithms to different parts of the inference problem. We then use this formalism to prove asymptotic convergence results for probablistic programs with inference metaprogramming. To the best of our knowledge this is the first asymptotic convergence result for hybrid probabilistic inference algorithms defined by (subproblem-based) inference metaprogramming.

==> language/completeness.tex <==
\Comment{
\begin{lemma}
    Given  a valid trace $t$, a valid subproblem $\cS$ and a valid trace $t'$, if
    $\SAC t \equiv t'$ then there exists a valid subproblem $\cS'$ on $t'$
    such that $\SAC t' \equiv t$, i.e.
    \[
        \cS \vdash t \equiv t' \implies \exists~\cS'.~ \cS' \vdash t' \equiv t
    \]
    and $\cS'$ is valid subproblem on $t'$.
\end{lemma}
%\input{language/proofcomp1.tex}

\begin{lemma}
The extraction process is the inverse of the stitching process i.e.
    Given two valid traces $t, t'$ and valid subproblems $\cS, \cS'$,
    s.t.
    \[
        \cS \vdash t \equiv t'~\wedge~\cS' \vdash t' \equiv t
    \]
    for any subtrace $t_s$:
    \[ t_s = \mathsf{ExtractTrace}(t', \cS') \implies
    t' = \mathsf{StitchTrace}(t, t_s, \cS) \]
\end{lemma}
\input{language/proofcomp2.tex}

\begin{lemma}
    Give two traces $t, t'$ and corresponding valid subproblems $\cS$ and 
    $\cS'$, such that
\begin{itemize}
\item $t' \in \mathsf{Trace}(\mathsf{Program}(t))$
\item $\SAC t \equiv t'$
\item $\cS' \vdash t' \equiv t$
\end{itemize}
then there exists $t_s$, $t'_s$ such that
    \begin{itemize}
        \item $t_s = \mathsf{ExtractTrace}(t, \cS)$
        \item $t'_s = \mathsf{ExtractTrace}(t', \cS')$
\end{itemize}
and $t'_s \in \mathsf{Traces}(\mathsf{Program}(t_s))$ 
    \label{lemma:comp-ex-p}
\end{lemma}


\begin{theorem}
    Given a valid trace $t$ and a valid subproblem $\cS$ and a subtrace 
    $t_s = \mathsf{ExtractTrace}(t, \cS)$. For all possible
    traces $t'$,
    \[
        t' \in \mathsf{Traces}(\mathsf{Program}(t))~\wedge~
    \SAC t \equiv t'\] 
    $\implies$

there exists a subtrace $t'_s$ such that
    \begin{itemize}
        \item $t'_s \in \mathsf{Trace}(\mathsf{Program}(t_s))$
        \item $t' = \mathsf{StitchTrace}(t, t'_s, \cS)$
     \end{itemize}
    \label{thm:complete}
\end{theorem}
\begin{proof}
Given a valid trace $t$ and a valid subproblem $\cS$, a subtrace $t_s = 
    \mathsf{ExtractTrace}(t, \cS)$, for all traces $t'$ such that 
    \begin{itemize}
        \item   $ t' \in \mathsf{Traces}(\mathsf{Program}(t)$
        \item $\SAC t \equiv t'$
    \end{itemize}
    we can define a valid subproblem of $\cS'$ such that 
    \[
        \SAC t' \equiv t
    \]
    we know that $t'_s = \mathsf{ExtractTrace}(t', \cS')$
    has the property
    \[
        t'_s \in \mathsf{Traces}(\mathsf{Program}(t_s))
    \]
    and 
    \[
        t' = \mathsf{StitchTrace}(t, t_s, \cS)
    \]

    Hence for all valid infered traces $t'$ there exist a 
    subtrace $t'_s$ which can give us $t'$.
\end{proof}
}

\input{language/proofcompsep.tex}



==> language/execution.tex <==
\[
 \mathsf{Dist}(e_v) \Rightarrow 
\]



==> language/infermeta.tex <==
\begin{figure}[h]
\[
\begin{array}{rcl}
c \in C &:=& b
            ~\vert~ \mathsf{infer}(\mathsf{SS}, c)  
            %~\vert~ \mathsf{If}(\mathsf{cond})\{~c~\}\\
            \\
            &\vert& \mathsf{If}(\mathsf{Bernoulli}(~p~))\{~c~\}
            ~\vert~ c_1;c_2\\
p_i \in P_i &:=& c
\end{array}
\]
    \caption{Inference Metaprogramming Language}
    \label{fig:infermetalang}
\end{figure}


==> language/proofcomp1.tex <==
\begin{proof}
We are going to define 
subproblem $\cS'$ using subproblem $\cS$.

\newcommand{\subprob} [1] {\mathsf{subproblem}\llbracket #1 \rrbracket}
    \[
        \subprob{\SAC \ndi{x}{x}{id} \equiv \ndi{x}{x}{id'}} = \begin{cases}
            \emptyset & id \notin \cS\\
            \{id'\} & id \in \cS\\
        \end{cases}
    \]
     \[
         \subprob{\SAC \ndi{x(id_v)}{v}{id} \equiv \ndi{x(id'_v)}{v'}{id'}} = \begin{cases}
            \emptyset & id \notin \cS\\
            \{id'\} & id \in \cS\\
        \end{cases}
    \]
     \[
        \subprob{\SAC \ndi{\lambda.x~e}{v}{id} \equiv \ndi{\lambda.x~e}{v'}{id'}} = 
            \emptyset
    \]
     \[
         \subprob{\SAC \ndi{\mathsf{Dist}(ae \#id_v )=ae_v}{v}{id} \equiv \ndi{\mathsf{Dist}(ae' \#id'_v) = ae'_v}{v'}{id'}} = \begin{cases}
            \emptyset & id \notin \cS\\
            \{id'\} & id \in \cS\\
        \end{cases}
    \]

    
    \[
        \subprob{\SAC \emptyset \equiv \emptyset} = \emptyset
    \]
    \[
        \begin{array}{c}
        \subprob{\SAC \assume{x}{ae};t \equiv \assume{x}{ae'};t'} =\\ \subprob{\SAC ae \equiv ae'}
        \bigcup \subprob{\SAC t \equiv t'}
        \end{array}
    \]
    \[
        \begin{array}{c}
        \subprob{\SAC \observed{ae}{e};t \equiv \observed{ae'}{e};t'} =\\ \subprob{\SAC ae \equiv ae'}
        \bigcup \subprob{\SAC t \equiv t'}
        \end{array}
    \]

\end{proof}


==> language/proofcomp2.tex <==
\begin{proof}
Proof by Induction.

For augmented expression $ae, ae'$ and valid subproblems $\cS$ and $\cS'$,
\[
\cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\wedge \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s \implies \cS \vdash ae, ae_s, t_s \Rightarrow_{st} ae', \emptyset
\]

\noindent{\bf Base Case:}

\noindent{\bf Case 1:} $ae = \ndi{x}{x}{id}, ae' = \ndi{x}{x}{id'}$.
Assuming
\[
\cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
$ae_s = \ndi{x}{x}{id'}$ and $t_s = \emptyset$.

The following is true
\[
\cS \vdash \ndi{x}{x}{id}, \ndi{x}{x}{id'}, \emptyset \Rightarrow_{st} ae'
\]


\noindent{\bf Case 2:} $ae = \ndi{x(id_v)}{v}{id}, ae' = \ndi{x(id'_v)}{v'}{id'}$.
Assuming
\[
\cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
$ae_s = \ndi{x(id'_v)}{v'}{id'}$ and $t_s = \emptyset$.

The following is true
\[
\cS \vdash \ndi{x(id_v)}{v}{id}, \ndi{x(id'_v)}{v'}{id'}, \emptyset \Rightarrow_{st} ae'
\]

\noindent{\bf Case 3:} $ae = \ndi{\lambda.x~e}{v}{id}, ae' = \ndi{\lambda.x~e}{v'}{id'}$.
Assuming
\[
\cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
$ae_s = \ndi{\lambda.x~e}{v'}{id'}$ and $t_s = \emptyset$.

The following is true
\[
\cS \vdash \ndi{\lambda.x~e}{v}{id}, \ndi{\lambda.x~e}{v'}{id'}, \emptyset \Rightarrow_{st} ae'
\]

\noindent{\bf Induction Cases:}

\noindent{Case 1:}
$ae = \ndi{(ae_1~ae_2)\perp}{v}{id}, ae' = \ndi{(ae'_1~ae'_2)\perp}{v'}{id'}$. Assuming from induction hypothesis
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \implies \cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \implies \cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Assuming 
\[
    \cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
$ae_s = \ndi{(ae^1_s~ae^2_s)}{v'}{id'}$ and $t_s = t^1_s;t^2_s$.
which implies 
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \]
is true, hence the following statements are true.
\[
\cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Hence 
\[
\cS \vdash \ndi{(ae_1~ae_2)\perp}{v}{id}, \ndi{(ae^1_s~ae^2_s)\perp}{v'}{id'}, t_s \Rightarrow_{st} ae'
\]


\noindent{Case 2:}
$ae = \ndi{(ae_1~ae_2)x=ae_3}{v}{id}, ae' = \ndi{(ae'_1~ae'_2)y=ae'_3}{v'}{id'}$ and $ID(ae_1) \in \cS$. Assuming from induction hypothesis
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \implies \cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \implies \cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Assuming 
\[
    \cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
as $ID(ae'_1) \in \cS'$,
$ae_s = \ndi{(ae^1_s~ae^2_s)y=ae'_3}{v'}{id'}$ and $t_s = t^1_s;t^2_s$.
which implies 
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \]
is true, hence the following statements are true.
\[
\cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Hence
$ID(ae_1) \in \cS$ 
\[
\cS \vdash \ndi{(ae_1~ae_2)x=ae_3}{v}{id}, \ndi{(ae^1_s~ae^2_s)y=ae'_3}{v'}{id'}, t_s \Rightarrow_{st} ae'
\]


\noindent{Case 3:}
$ae = \ndi{(ae_1~ae_2)y=ae_3}{v}{id}, ae' = \ndi{(ae'_1~ae'_2)y=ae'_3}{v'}{id'}$ and $ID(ae_1) \notin \cS$. Assuming from induction hypothesis
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \implies \cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \implies \cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]
\[
\cS \vdash ae_3 \equiv ae'_3 \wedge \cS' \vdash ae'_3 \equiv ae_3
\wedge \cS' \vdash ae'_3 \Rightarrow_{ex} ae^3_s, t^3_s \implies \cS \vdash ae_3, ae^3_s, t^3_s \Rightarrow_{st} ae'_3, \emptyset
\]

Assuming 
\[
    \cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
as $ID(ae'_1) \notin \cS'$,
$ae_s = \ndi{ae^3_s}{v'}{id'}$ and $t_s = t^1_s;\assume{x}{ae^1_s};t^2_s;\assume{y}{ae^2_s};t^3_s$.
which implies 
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \]
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \]
\[
\cS \vdash ae_3 \equiv ae'_3 \wedge \cS' \vdash ae'_3 \equiv ae_3
\wedge \cS' \vdash ae'_3 \Rightarrow_{ex} ae^3_s, t^3_s \]
is true, hence the following statements are true.
\[
\cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
\[
\cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]
\[
\cS \vdash ae_3, ae^3_s, t^3_s \Rightarrow_{st} ae'_3, \emptyset
\]

Hence
\[
\cS \vdash \ndi{(ae_1~ae_2)x=ae_3}{v}{id}, \ndi{ae'_3}{v'}{id'}, t_s \Rightarrow_{st} ae'
\]


\noindent{Case 4:}
$ae = \ndi{\mathsf{Dist}(ae_1\#id_e) = ae_2}{v}{id}, ae' = \ndi{\mathsf{Dist}(ae'_1\#id_e) = ae'_2}{v'}{id'}$ and $id_e \notin \cS$. Assuming from induction hypothesis
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \implies \cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \implies \cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Assuming 
\[
    \cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
as $id_e \notin \cS'$,
$ae_s = \ndi{ae^2_s}{v'}{id'}$ and $t_s = t^1_s;\observed{ae^1_s}{e};t^2_s$, $ae^2_s \Rightarrow_r e$.
which implies 
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \]
and 
\[
\cS \vdash ae_2 \equiv ae'_2 \wedge \cS' \vdash ae'_2 \equiv ae_2
\wedge \cS' \vdash ae'_2 \Rightarrow_{ex} ae^2_s, t^2_s \]
is true, hence the following statements are true.
\[
\cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]
and 
\[
\cS \vdash ae_2, ae^2_s, t^2_s \Rightarrow_{st} ae'_2, \emptyset
\]

Hence
$id_e \notin \cS$ 
\[
\cS \vdash ae, ae_s, t_s \Rightarrow_{st} ae'
\]


\noindent{Case 5:}
$ae = \ndi{\mathsf{Dist}(ae_1\#id_e) = ae_2}{v}{id}, ae' = \ndi{\mathsf{Dist}(ae'_1\#id'_e) = ae'_2}{v'}{id'}$ and $id_e \in \cS$. Assuming from induction hypothesis
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \implies \cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]

Assuming 
\[
    \cS \vdash ae \equiv ae' \wedge \cS' \vdash ae' \equiv ae
\]
\[
    \cS' \vdash ae' \Rightarrow_{ex} ae_s, t_s
\]
as $id_e \notin \cS'$,
$ae_s = \ndi{\mathsf{Dist}(ae^1_s\#i'd_e) = ae'_2}{v'}{id'}$ and $t_s = t^1_s$.
which implies 
\[
\cS \vdash ae_1 \equiv ae'_1 \wedge \cS' \vdash ae'_1 \equiv ae_1
\wedge \cS' \vdash ae'_1 \Rightarrow_{ex} ae^1_s, t^1_s \]
and 
is true, hence the following statements are true.
\[
\cS \vdash ae_1, ae^1_s, t^1_s \Rightarrow_{st} ae'_1, \emptyset
\]

Hence
$id_e \in \cS$ 
\[
\cS \vdash ae, ae_s, t_s \Rightarrow_{st} ae'
\]

Hence the statement is true for augmented expressions.

For any two traces $t, t'$ and any two subproblems $\cS$ and $\cS'$
\[
    S
\]



\end{proof}


==> language/subproblem.tex <==
\section{Valid Subproblem}
Given a trace $t$ with the dependence graph 
$\NDE{}{}{} = \mathsf{Graph}(t)$ a valid subproblem $\cS \subseteq \dom \cN$
must satisfy two properties: 1) there are no outgoing existential edges and
2) all outgoing data dependence edge must terminate at a 
stochastic choice ($\mathsf{Sample}$ node).


\begin{itemize}
\item $\forall id \in \cS.~\tup{id, id_o} \in \cE  \implies id_o \in \cS$
\item  $\forall id \in \cS.~\tup{id, id_o} \in \cD \wedge id_o \in \dom \cN 
- \cS \implies \cN(id_o) = \mathsf{Sample} $
\end{itemize}

The absorbing set $\cA \subseteq \dom \cN - \cS$ of a subproblem $\cS$ 
is the set of stochastic choices whose value directly depends on the 
nodes in the subproblem i.e. $\cA = \{id_a \vert id_a \in \dom \cN
- \cS \wedge \exists~id_i \in \cS.~\tup{id_i, id_o} \in \cD\}$.

Since given a trace $t$ and a valid subproblem $\cS$, an absorbing set 
$\cA$ is naturally defined, from this point on we will call the tuple 
$\cS, \cA$ as a valid subproblem for trace $t$.


==> language/trace-monad.tex <==
\[

\]

\begin{figure*}
\[
\begin{array}{c}
\end{array}
\]
\end{figure*}


==> language/traces-from-same-prog.tex <==

\begin{figure*}
    \begin{subfigure}{\textwidth}
    \[
\begin{array}{c}
%    \begin{array}{ccc}
    \begin{array}{cc}
    \infral{
        \Unid{id, id'}\\
        x \notin \dom \sigma_v~~~~~x \notin \dom \sigma'_v\\
    }
        {\SII{}{}{'}{'} \ndi{x}{x}{id} \equiv_p \ndi{x}{x}{id'} }{VAR}
    &
    \infral{
        \Unid{id, id'}\\
        v_1 = \sigma_v(x) ~~~~~~
        id_1 = \sigma_{id}(x) ~~~~~
        v_2 = \sigma'_v(x)~~~~~~
        id_2 = \sigma'_{id}(x)\\
    }
        {\SII{}{}{'}{'} \ndi{x(id_1)}{v_1}{id} \equiv_p \ndi{x(id_2)}{v_2}{id'} }
        {VAR-ASSIGN}
    \end{array}
        %&
    \\
    \\
    \infral{
        \Unid{id, id'}\\
        \sigma''_v = \mathsf{RestrictKeys}(\sigma_v, \mathsf{FreeVariables}(\lambda.x~e)) ~~~~~~
        \sigma'''_v = \mathsf{RestrictKeys}(\sigma'_v, \mathsf{FreeVariables}(\lambda.x~e))\\ 
        \sigma''_{id} = \mathsf{RestrictKeys}(\sigma_{id}, \mathsf{FreeVariables}(\lambda.x~e)) ~~~~~~
        \sigma'''_{id} = \mathsf{RestrictKeys}(\sigma'_{id}, \mathsf{FreeVariables}(\lambda.x~e))\\
    }
    {\SII{}{}{'}{'} \ndi{\lambda.x~e}{
        \tup{\lambda.x~e, \sigma''_v, \sigma''_{id}} }{id} 
    \equiv_p   \ndi{\lambda.x~e}{
        \tup{\lambda.x~e, \sigma'''_v, \sigma'''_{id}} }{id}   }{LAM}
    %\end{array}
    \\
    \\
    \infral{
        \Unid{id, id'}\\
        \SII{}{}{'}{'} ae_1 \equiv_p ae'_1
        ~~~~~~~~~~~~~
    \SII{}{}{'}{'} ae_2 \equiv_p ae'_2  ~~~~~~
    ae_1 \Rightarrow_r e_1 ~~~~~~ ae_2 \Rightarrow_r e_2\\
    \SI{}{} (e_1~e_2) \Rightarrow_s v, id, \ndi{(ae_1~ae_2)aa}{v}{id} ~~~~~~    
    \SI{'}{'} (e_1~e_2) \Rightarrow_s v', id', \ndi{(ae'_1~ae'_2)aa'}{v'}{id'}\\
    %\cV(ae'_1) = \tup{\lambda.x~e, \sigma'_v, \sigma'_{id}}\\
        %\SI{'[x \rightarrow \cV(ae'_2)]}{'[x \rightarrow \ID(ae'_2)]} 
        %e \Rightarrow_s v, id_e, ae'_3\\
    }
    {\SII{}{}{'}{'} \ndi{(ae_1~ae_2)aa}{v}{id} \equiv_p 
     \ndi{(ae'_1~ae'_2)aa'}{v'}{id'} }{APP}
    \\    \\
    \infral{
        \Unid{id, id', id_e, id'_e}\\
        \SII{}{}{'}{'} ae \equiv_p ae'
        ~~~~~~~~~~
        ae_v \Rightarrow_r e_v
        ~~~~~~
        ae'_v \Rightarrow_r e'_v ~~~~~~
        e_v \in \dom \mathsf{Dist}(\cV(ae))
        ~~~~~~~~
        e'_v \in \dom \mathsf{Dist}(\cV(ae'))\\
        \SI{}{} e_v \Rightarrow_s v, id_v, ae_v
        ~~~~~
        \SI{'}{'} e'_v \Rightarrow_s v', id'_v, ae'_v\\
    }
        {\SII{}{}{'}{'} \ndi{\mathsf{Dist}(ae\#id_e) = ae_v}{v}{id} \equiv_p 
      \ndi{\mathsf{Dist}(ae'\#id'_e)=ae'_v}{v'}{id'} }{DIST}
    %\end{array}
    \end{array}
    \]
    \caption{Check for 2 augmented expressions ,$\equiv_p \subseteq \Sigma_v \times \Sigma_{id} \times aE \times aE$ }
\end{subfigure}
\begin{subfigure}{\textwidth}
    \[
        \begin{array}{cc}
    \infral{}
            {\SII{}{}{'}{'} \emptyset \equiv_p \emptyset}{BASE}
    &
            \begin{array}{c}
    \infral{
        \SII{}{}{'}{'} ae \equiv_p ae'\\
        \SII{[x \rightarrow \cV(ae)]}{[x \rightarrow \ID(ae)]}
            {'[x \rightarrow \cV(ae')]}{'[x \rightarrow \ID(ae')]}
            t \equiv_p t'\\
    }
            {\SII{}{}{'}{'} \assume{x}{ae};t \Rightarrow_p \assume{x}{ae'};t' }
            {ASSUME}
                \\
            \\
    \infral{
        \Unid{id, id'}\\
            \SII{}{}{'}{'} ae \equiv_p ae' ~~~~~~
            \SII{}{}{'}{'} t \equiv_p t'\\
    }
            {\SII{}{}{'}{'} \observed{ae\#id}{e_v};t \equiv_p \observed{ae'\#id'}{e_v};t'}
                {OBSERVE}
            \end{array}
        \end{array}
\]
    \caption{Check over given traces , $\equiv_p \subseteq \Sigma_v \times \Sigma_{id} \times T \times T$}
\end{subfigure}
\caption{Traces from same program}
\label{fig:tracesfromsameprog}
\end{figure*}



==> test <==
Convergence of inference algorithms has been well studied in math and statistics~\cite{XXX, XXX, XXX}.
These 

